Doing Experiments and Revising Rules with Natural Language and Probabilistic Reasoning

We give a model of how to infer natural language rules by doing experiments. The model integrates Large Language Models (LLMs) with Monte Carlo algorithms for probabilistic inference, interleaving online belief updates with experiment design under information-theoretic criteria. We conduct a human-model comparison on a Zendo-style task, finding that a critical ingredient for modeling the human data is to assume that humans also consider fuzzy, probabilistic rules, in addition to assuming that humans perform approximately-Bayesian belief updates. We also compare with recent algorithms for using LLMs to generate and revise hypotheses, finding that our online inference method yields higher accuracy at recovering the true underlying rule, and provides better support for designing optimal experiments.

==> figs/45plots.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=\linewidth]{imgs/full_45plots.pdf}
\vspace{-2em}
\caption{Comparing human and model accuracy on the 8 test scenes after 7 rounds of experimentation with breakdowns for the 4 rule-following (RF) and 4 not rule-following (Not RF) test scenes. The rows and columns of the grid of plots are the methods and the 9 rules respectively. Online inference with fuzzy rules, presented in the last row, most closely matches the accuracy breakdown observed in humans.}
\vspace{-0.8em}
\label{fig:45plots}
\end{figure*}

==> figs/initial_prompts.tex <==
\begin{figure*}[!h]
\centering
\hrulefill

\texttt{
You are playing an inductive game with me. I'll be the moderator, and your task is to figure out the secret rule that I know by coming up with a structure of blocks to ask me whether it conforms with the secret rule or not. 
\\
The structure has one of more blocks. Each block should contain the following attributes: 
color (blue/red/green) 
size (small/medium/large)
orientation (upright/left/right/strange)
groundedness (grounded/ungrounded),
touching (which other blocks they do and do not touch).
\\
To give you a start, I'll describe one structure that follows the rule:
\\
\{text\_c\}
\\
Give a very short summary on what you currently think the secret rule is.
}

\hrulefill
\caption{Prompt used for roleplaying Vanilla LLM}
\label{fig:prompt_vanilla}
\end{figure*}

==> figs/learnability_and_logl.tex <==
\begin{figure}[ht]
\centering
\begin{minipage}{0.5\textwidth}
\centering
\begin{tabular}{c@{\hspace{5pt}}c}
\toprule
Method & LogL   \\
\midrule
Bramley et al. \cite{bramley2018grounding}’s best model                          & \textasciitilde$-1385.10^*$         \\
Batch, Fuzzy               & $-1520.86$        \\
Online, Fuzzy              & $\bm{-1334.75}$        \\
Batch, Hard                & $-2845.40$        \\
Batch w/ Refinement, Hard & $-2951.68$  \\
Online, Hard               & $-4590.30$        \\
\bottomrule
\end{tabular}
\captionof{table}{hi}
\end{minipage}\hfill
\begin{minipage}{0.5\textwidth}
\centering
\includegraphics[width=\linewidth]{imgs/majority_is_red.pdf} % example image
\caption{Sample Figure}
\end{minipage}
% \hfill
% \begin{minipage}{0.33\textwidth}
% \centering
% \includegraphics[width=\linewidth]{imgs/r2-cost.pdf} % example image
% \caption{Sample Figure}
% \end{minipage}
\end{figure}

==> figs/learnability_and_logl_and_r2_cost.tex <==
\begin{figure}[ht]
\centering
\begin{minipage}{0.32\textwidth}
\centering
\tiny{
\begin{tabular}{cc}
\toprule
Method & LogL   \\
\midrule
Bramley et al. \cite{bramley2018grounding}’s best model                          & \textasciitilde$-1385.10^*$         \\
Batch, Fuzzy               & $-1520.86$        \\
Online, Fuzzy              & $\bm{-1334.75}$        \\
Batch, Hard                & $-2845.40$        \\
Batch w/ Refinement, Hard & $-2951.68$  \\
Online, Hard               & $-4590.30$        \\
\bottomrule
\end{tabular}}
\captionof{table}{hi}
\end{minipage}\hfill
\begin{minipage}{0.33\textwidth}
\centering
\includegraphics[width=\linewidth]{imgs/majority_is_red.pdf} % example image
\caption{Sample Figure}
\end{minipage}
\hfill
\begin{minipage}{0.33\textwidth}
\centering
\includegraphics[width=\linewidth]{imgs/r2-cost.pdf} % example image
\caption{Sample Figure}
\end{minipage}
\end{figure}

==> figs/r2.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.32\linewidth]{imgs/r2_full_direct_llm.pdf}
\includegraphics[width=0.32\linewidth]{imgs/r2_full_is_det.pdf}
\includegraphics[width=0.32\linewidth]{imgs/r2_full_is_refine_det.pdf}
\includegraphics[width=0.32\linewidth]{imgs/r2_full_particle_filter_det.pdf}
\includegraphics[width=0.32\linewidth]{imgs/r2_full_is.pdf}
\includegraphics[width=0.32\linewidth]{imgs/r2_full_particle_filter.pdf}
\caption{Human vs model accuracy after 7 rounds of experimentation. Each point is a different rule assessed either on structures that follow or do not follow the rule ($\pm$RF). Removing even a single component of the model significantly degrades its ability to predict human accuracy.}
\vspace{-0.8em}
\label{fig:r2}
\end{figure*}

==> figs/r2_cost.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{imgs/full-r2-cost.pdf}
\caption{\Top{TODO}}
% \vspace{-0.8em}
\label{fig:r2_cost}
\end{figure*}

==> figs/r2_lower_small_and_logl.tex <==
\begin{figure}
\begin{minipage}[b]{.65\linewidth}
\centering
\includegraphics[width=0.49\linewidth]{imgs/r2_lower_full_is.pdf}
\includegraphics[width=0.49\linewidth]{imgs/r2_lower_full_particle_filter.pdf}
\caption{R2 at test scene level (small) \Top{TODO}. See the full version at \Cref{fig:r2_lower}} 
\label{fig:r2_lower_small}
\end{minipage}\hfill
\begin{minipage}[b]{.32\linewidth}
\centering
\adjustbox{max width=\textwidth}{
\centering
\setlength\tabcolsep{4pt} % control the horizontal spacing between columns
\begin{tabular}{c@{\hspace{5pt}}c}
\toprule
Method & LogL   \\
\midrule
Bramley’s best model                           & \textasciitilde$-1385.10^*$         \\
Batch, Fuzzy               & $-1520.86$        \\
Online, Fuzzy              & $\mathbf{-1334.75}$        \\
Batch, Hard                & $-2845.40$        \\
Batch w/ Refinement, Hard & $-2951.68$  \\
Online, Hard               & $-4590.30$        \\
\bottomrule
\end{tabular}}
\caption{LogL \Top{TODO}sdfsdf sdf}
\label{tab:logl}
\end{minipage}
\end{figure}

==> old_figs/accuracy.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.49\linewidth]{imgs/rule-following.pdf}
\includegraphics[width=0.49\linewidth]{imgs/not-rule-following.pdf}
\caption{(UPDATE PLS) Accuracy between models and human. RF means rule following and Not RF means not rule following.}
\label{fig:accuracy}
\end{figure*}

==> old_figs/inference_alg.tex <==
\begin{algorithm*}[t]
\caption{online SMC-like inference algorithm}\label{inference-alg}
\begin{algorithmic}
\State Let $(x_1, y_1)$ be the first data point we observe
\State $h_1^{(1)}, ..., h_1^{(n)} \sim q(h|x_1, y_1)$
\State $w_1^{(i)} \gets p(h_1^{(i)})$ for $1 \leq i \leq n$ \Comment{set initial particle weights}
\State $\theta_1^{(i)} \gets \argmax_\theta p(x_1, y_1, h_1^{(i)}, \theta)$ for $1 \leq i \leq n$ \Comment{set $\theta$s to their MAP estimates}
\State $(H_1, W_1) \gets \textit{Resampling}(H_1, W_1)$ \Comment{resampling}

\For{$t = 2, ..., T$}
\State The active learning algorithm gives $(x_t, y_t)$
\State $\theta_t^{(i)} \gets \argmax_\theta p(X, Y, h_t^{(i)}, \theta)$ for $1 \leq i \leq n$ \Comment{set $\theta$s to their MAP estimates}
\State $w_t^{(i)} \gets w_{t-1}^{(i)} \cdot p(y_t|x_t, h_t^{(i)}, \theta_{t}^{(i)}) \cdot \frac{p(X, Y, h_t^{(i)}, \theta_{t}^{(i)})}{p(X, Y, h_t^{(i)}, \theta_{t-1}^{(i)})}$ for $1 \leq i \leq n$ \Comment{data reweighting and theta reweighting}
\State $(H_t, \Theta_t, W_t) \gets \textit{Rejuvenation}(H_t, \Theta_t, W_t, X, Y, t)$ \Comment{rejuvenation with budget}
\State $(H_t, W_t) \gets \textit{Resampling}(H_t, W_t)$ \Comment{resampling}
\EndFor
\end{algorithmic}
\end{algorithm*}

==> old_figs/new_rejuvenation_step.tex <==
\begin{algorithm*}[t]
\caption{NEW Rejuvenation step}\label{rejuvenation-step}
\begin{algorithmic}
\Function{Rejuvenation}{$H, \Theta, W, x_{1:t}, y_{1:t}, t$}
\State $J \gets sort\_indices(\{p(h^{(i)}, \theta^{(i)}|x_{1:t}, y_{1:t}))\}_{i=1}^n$ \Comment{Sorts the posterior and returns sorted indices array $J$}

\For{$j \in J$}
\If{there is still budget left to sample from $q(h|h^{(j)}, x_t, y_t)$ }
    \State $h_{local}^{(1)}, ..., h_{local}^{(K)} \sim q(h|h^{(j)}, x_t, y_t)$ \Comment{Local sampling}
    \State $\theta_{local}^{(i)} \gets \argmax_\theta p(x_{1:t}, y_{1:t}, h_{local}^{(i)}, \theta)$ for $1 \leq i \leq n$ \Comment{Theta estimation}
    \State $v_i \gets \frac{p(h_{local}^{(i)},\theta_{local}^{(i)}|x_{1:t}, y_{1:t})}{q(h_{local}^{(i)}|h^{(j)}, x_t, y_t)}$ for $1 \leq i \leq n$ \Comment{Set sampling weights}
    \State ($h^{(j)}, \theta^{(j)}) \gets$ sample from $(H_{local}, \Theta_{local})$ with probability directly proportional to $v_{1:K}$
    \State $w^{(j)} \gets w^{(j)} \cdot \frac{1}{K \cdot p(h^{(j)},\theta^{(j)}|x_{1:t}, y_{1:t})} \cdot (\sum_{i=1}^K \frac{p(h_{local}^{(i)},\theta_{local}^{(i)}|x_{1:t}, y_{1:t})}{q(h_{local}^{(i)}|h^{(j)}, x_t, y_t)})$ \Comment{Update weight}
\EndIf
\EndFor 

\Return $H, \Theta, W$

\EndFunction
\end{algorithmic}
\end{algorithm*}

==> old_figs/rejuvenation_step.tex <==
\begin{algorithm*}[t]
\caption{Rejuvenation step}\label{rejuvenation-step}
\begin{algorithmic}
\Function{Rejuvenation}{$H, \Theta, W, X, Y, t$}
\State $J \gets sort\_indices(\{p(X, Y, h^{(i)}, \theta^{(i)}))\}_{i=1}^n$ \Comment{Sorts the joint likelihood and returns sorted indices array $J$}

\For{$j \in J$}
\If{there is still budget left for sampling from $q(h|h^{(j)}, x_t, y_t)$ }
    \State $h_{local}^{(1)}, ..., h_{local}^{(k)} \sim q(h|h^{(j)}, x_t, y_t)$ \Comment{sample local move proposals}
    \State $\theta_{local}^{(i)} \gets \argmax_\theta p(X, Y, h_{local}^{(i)}, \theta)$ for $1 \leq i \leq n$ \Comment{set $\theta$s to their MAP estimates}
    \State $H_{local}, \Theta_{local} \gets \{(h_{local}^{(i)}, \theta_{local}^{(i)}) \mid p(X, Y, h_{local}^{(i)}, \theta_{local}^{(i)}) > p(X, Y, h^{(j)}, \theta^{(j)})\}$ \Comment{filter out bad proposals}
    \If{$|H_{local}| > 0$} \Comment{we make the move if there are good proposals}
        \State $(h_{original}, \theta_{original}) \gets (h^{(j)}, \theta^{(j)})$
        \State ($h^{(j)}, \theta^{(j)}) \gets$ sample from $(H_{local}, \Theta_{local})$ with probability directly proportional to $\{p(X, Y, h_{local}^{(i)}, \theta_{local}^{(i)}))\}_{i=1}^m$
        \State $w^{(j)} \gets w^{(j)} \cdot \frac{p(y_t|x_t, h^{(j)},\theta^{(j)})}{p(y_t|x_t, h_{original}, \theta_{original})}$
    \EndIf
\EndIf
\EndFor 

\Return $H, \Theta, W$

\EndFunction
\end{algorithmic}
\end{algorithm*}

==> tables/active_learning_ablation.tex <==
\begin{table*}[t]
\centering
\adjustbox{max width=\textwidth}{
\centering
\setlength\tabcolsep{4pt} % control the horizontal spacing between columns
\begin{tabular}{c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}c@{\hspace{5pt}}}
\toprule
Active learning method & \multicolumn{2}{c}{Inference method}\\ 
\cmidrule(lr){2-3}
& Online, Fuzzy & Online, Hard \\
\midrule
LLM                            & $4.52 \pm 0.08$                            & $4.72 \pm 0.08$                            \\
Random                          & $5.03 \pm 0.11$                            & $5.84 \pm 0.19$                            \\
Info Gain       & $\bm{5.35 \pm 0.09}$                            & $\bm{6.55 \pm 0.13}$\\             
\bottomrule
\end{tabular}}
\caption{\Top{todo}}
% \vspace{-3pt}
\label{tab:active}
\end{table*}

==> tables/logl.tex <==
\begin{table*}[t]
\centering
\adjustbox{max width=\textwidth}{
\centering
\setlength\tabcolsep{4pt} % control the horizontal spacing between columns
\begin{tabular}{c@{\hspace{5pt}}c}
\toprule
Method & LogL   \\
\midrule
Bramley et al. \cite{bramley2018grounding}’s best model                          & \textasciitilde$-1385.10^*$         \\
Batch, Fuzzy               & $-1520.86$        \\
Online, Fuzzy              & $\bm{-1334.75}$        \\
Batch, Hard                & $-2845.40$        \\
Batch w/ Refinement, Hard & $-2951.68$  \\
Online, Hard               & $-4590.30$        \\
\bottomrule
\end{tabular}}
\caption{LogL \Top{TODO}}
\label{tab:logl}
\end{table*}

==> tables/proposer_ablation.tex <==
\begin{table*}[t]
\centering
\adjustbox{max width=\textwidth}{
\centering
\setlength\tabcolsep{4pt} % control the horizontal spacing between columns
\begin{tabular}{ccccc}
\toprule
Proposer for Info Gain & \multicolumn{3}{c}{Number of candidate experiments}\\ 
\cmidrule(lr){2-4}
& 1 & 5 & 10 \\
\midrule
Random proposer & $5.84 \pm 0.19$ & $6.23 \pm 0.16$ & $6.55 \pm 0.28$ \\
LLM proposer   &   $5.73 \pm 0.16$ & $6.19 \pm 0.12$           & $6.55 \pm 0.13$           \\
\bottomrule
\end{tabular}}
\caption{\Top{todo}}
% \vspace{-3pt}
\label{tab:proposer}
\end{table*}
